Sparse Stochastic Bandits

In the classical multi-armed bandit problem, d arms are available to the decision maker who pulls them sequentially in order to maximize his cumulative reward. Guarantees can be obtained on a relative quantity called regret, which scales linearly with d (or with sqrt(d) in the minimax sense). We here consider the sparse case of this classical problem in the sense that only a small number of arms, namely s < d, have a positive expected reward. We are able to leverage this additional assumption to provide an algorithm whose regret scales with s instead of d. Moreover, we prove that this algorithm is optimal by providing a matching lower bound - at least for a wide and pertinent range of parameters that we determine - and by evaluating its performance on simulated data.

==> LowerBound.tex <==
%!TEX root = main_colt.tex
%


%\subsection{Version 2 : For a given sparsity level $\epsilon$}
This section is devoted to proving a lower bound on the regret of any \emph{uniformly efficient } algorithm for the sparse bandit problem. Our goal is to provide a result that is easily generalizable to any stochastic bandit problem containing a sparsity information in the form of a threshold on the values of the expected return of the arms of interest. A generalization of the presented bound can be found in Appendix \ref{ap:LB2}.

For the sake of completeness, we briefly recall the following definition as stated in \cite{lai1985asymptotically}:
\begin{definition}
	\label{def:uniformly_eff}
	An algorithm is \emph{uniformly efficient} if for any sparse
	bandit problem and all $\alpha\in(0,1]$, its expected regret satisfies
	$\mathbb{E}\left[   \operatorname{Reg}(T) \right] = o(T^\alpha)$.
\end{definition}


%In this section, we give a problem-dependent lower bound on the regret of any
%\emph{uniformly efficient} algorithm for the sparse bandit problem.

For the sake of clarity, we state the bound for Gaussian bandit models with a 
fixed variance equal to $1/4$. In that case, a distribution is simply 
characterized by its mean $\mu$ and the Kullback-Leibler (KL) divergence between 
two models $\mu$ and $\mu'$ is equal to $2(\mu-\mu')^2$.

%\subsection{A general Problem-Dependent Lower Bound}
\begin{theorem}
	\label{cor:LB}
	For a Gaussian sparse bandit problem $\nu =
	(\nu_1,\ldots,\nu_s,\nu_{s+1},\ldots,\nu_d) \in
	\mathcal{S}(d,s)\in \mathbb{R}^d$, an asymptotic lower bound on 
	the regret is given by the solution to the following linear optimization 
	problem:
	\begin{eqnarray}
	&  & f(\mu)\geq \quad \inf_{c\succeq 0} c_i \Delta_i\\
	s.t. & \quad\forall i\in \{2,...,s\},
	& 2 c_i \Delta_i^2\geq 1;\\
	& \forall i\in \{2,\ldots,s\},\, \forall j\in \{s+1,...d\},  & 2 c_j 
	\mu_1^2+ 2 c_i \mu_i^2 \geq 1\\
	& \forall i\in \{1,\ldots,d\}, & c_i \geq 0
	\end{eqnarray}
	whose solution can be computed explicitly and gives the following 
	problem-dependent lower bound:
	\begin{itemize}
		\item If $\frac{d-s}{\mu_1}- 
			\sum_{\substack{i\in [s]\\\Delta_i>0}}^{}\frac{\Delta_i}{\mu_i^2} > 0$,
		\begin{equation}
		\label{cor:LB0}
		\liminf_{T\to \infty}\frac{\operatorname{Reg}(T)}{\log(T)} \geq \sum_{\substack{i\in [s]\\\Delta_i>0}}^{}\max\Big\{ \frac{1}{2\Delta_i},\frac{\Delta_i}{2\mu_i^2}\Big\}
		\end{equation}
		\item otherwise, there exist $k\leq s$ such that $\frac{d-s}{\mu_1}- 
		\sum_{i=k}^{s}\frac{\Delta_i}{\mu_i^2} < 0$, and the lower bound is 
		\begin{equation}
		\label{cor:LB1}
		\liminf_{T\to \infty}\frac{\operatorname{Reg}(T)}{\log(T)} \geq \sum_{\substack{i\in [k]\\\Delta_i>0}}^{} 
		\frac{1}{2\Delta_i} + \sum_{i=k+1}^{s} 
		\frac{\mu_{k}^2}{\mu_i^2}\frac{\Delta_i}{2\Delta_{k}^2}
		+\frac{(d-s)}{2\mu_1}
		\left(1-\frac{\mu_{k}^2}{\Delta_{k}^2}\right).
		\end{equation}
	\end{itemize}

\end{theorem}

% \begin{corollary} 
% \label{cor:LB}
% 	When the sparsity gap exactly matches the considered sparse 
% bandit problem, that is when $\epsilon = \mu_s$, the lower bound of 
% Theorem~\ref{th:LB2} is simply 
% \begin{equation}
% \label{cor:LB0}
% \liminf_{T\to \infty}\frac{\operatorname{Reg}(T)}{\log(T)} \geq \sum_{\substack{i\in [s]\\\Delta_i>0}}^{}\max\Big\{ \frac{1}{2\Delta_i},\frac{\Delta_i}{2\mu_i^2}\Big\}
% \end{equation}
% in the first case. In the second case, it becomes
% \begin{equation}
% \label{cor:LB1}
% \liminf_{T\to \infty}\frac{\operatorname{Reg}(T)}{\log(T)} \geq \sum_{\substack{i\in [k]\\\Delta_i>0}}^{} 
% \frac{1}{2\Delta_i} + \sum_{i=k+1}^{s} 
% \frac{\mu_{k}^2}{\mu_i^2}\frac{\Delta_i}{2\Delta_{k}^2}
% +\frac{(d-s)}{2\mu_1}
% \left(1-\frac{\mu_{k}^2}{\Delta_{k}^2}\right).
% \end{equation}
% \end{corollary}

\textbf{Remarks.} Since the decision maker has more knowledge on the parameters of the problem than in the classical multi-armed bandit problem, we expect the lower bound to be less than the traditional one (without the sparsity assumption), which is 
$$
\liminf_{T\to \infty}\frac{\operatorname{Reg}(T)}{\log(T)} \geq \sum_{\substack{i\in [d]\\\Delta_i>0}}^{} \frac{1}{2\Delta_i}\ .
$$
Indeed, since the $\max$ is smaller than the sum, in the first case, we have
$$ \sum_{\substack{i\in [s]\\\Delta_i>0}}^{}\max\Big\{ \frac{1}{2\Delta_i},\frac{\Delta_i}{2\mu_i^2}\Big\} \leq  \sum_{\substack{i\in [s]\\\Delta_i>0}}^{} \frac{1}{2\Delta_i} + \sum_{\substack{i\in [s]\\\Delta_i>0}}^{} \frac{\Delta_i}{2\mu_i^2}\leq   \sum_{\substack{i\in [s]\\\Delta_i>0}}^{} \frac{1}{2\Delta_i} +\frac{d-s}{\mu_1}= \sum_{\substack{i\in [d]\\\Delta_i>0}}^{} \frac{1}{2\Delta_i}\ .
$$
Similarly, in the second case, we get that
\begin{align*}
 \sum_{i=1}^{k} 
\frac{1}{2\Delta_i} + \sum_{i=k+1}^{s} 
\frac{\mu_{k}^2}{\mu_i^2}\frac{\Delta_i}{2\Delta_{k}^2}  +\frac{(d-s)}{2\mu_1}\left(1-\frac{\mu_{k}^2}{\Delta_{k}^2}\right) & =
 \sum_{\substack{i\in [d]\\\Delta_i>0}}^{} \frac{1}{2\Delta_i} - \frac{\mu_k^2}{\Delta_k^2}\Big(\underbrace{\frac{d-s}{2\mu_1}-\sum_{i=k+1}^s \frac{\Delta_i}{2\mu_i^2}}_{> 0}\Big)-\sum_{i=k+1}^s \frac{1}{2\Delta_i} .
\end{align*}
Moreover, if $\frac{\Delta_s}{\mu_s^2} > \frac{d-s}{\mu_1}$, then both lower bound match. Stated otherwise, the sparsity assumption is irrelevant as soon as
$$
\mu_s \leq \mu_1 \frac{-1 + \sqrt{1+4(d-s)}}{2(d-s)} \simeq \frac{\mu_1}{\sqrt{d-s}}\ .
$$

\begin{proof}
	The proof relies on changes of measure arguments originating from \cite{graves1997asymptotically}.
	First, consider the set of changes of distributions that modify the
	best arm without changing the marginal of the best arm in the original 
	sparse bandit
	problem. Namely, for a given $\mu\in \mathcal{S}(d,s)$, we consider the
	following set of acceptable changes of measure
	\[
	\mathcal{B}(\mu) = \{\mu' \in \mathcal{S}(d,s) \,\vert\, \mu'_1 = \mu_1,
	\max_i \mu_i < \max_i \mu'_i \}.
	\]
	
	Concretely, if one considers an alternative sparse bandit model $\mu'$ such 
	that  one
	of the originally null arms becomes the new best arm, then one of the
	originally non-null arms in $\mu$ must be taken to zero in $\mu'$ in order 
	to keep the
	spare structure of the problem.
	In general, the equivalent of Th.~17 in \citep{kaufmann2015complexity}
	or Proposition~3 in \citep{lagree2016multiple} can be stated in our case
	as follows: For all changes of measure $\mu' \in \mathcal{B}(\mu)$,

	\begin{equation}
	\label{eq:constraint}
	\liminf_{T\to \infty} \dfrac{\sum_{i=1}^{d} 2 \mathbb{E}
		[N_i(T+1)](\mu_i-\mu'_i)^2}{\log(T)} \geq 1.  	
	\end{equation}
	Details on this type of informational lower bounds can be found in \cite{garivier2016explore} and references therein.
	
	Now, following general ideas from \cite{graves1997asymptotically} and
	lower bound techniques from
	\cite{lagree2016multiple} and \cite{combes2015combinatorial}, we may give a
	variational form of the lower bound on the regret satisfying the above 
	constraint.
	
	\begin{eqnarray}
	\label{eq:opt_problem}
	\liminf_{T\rightarrow \infty} \frac{\operatorname{Reg}(T)}{\log (T)}  \geq f(\mu) &
	\text{\emph{where},} &  \quad  f(\mu) = \inf_{c\succeq 0} c_i
	\Delta_i  \\
	& & \qquad s.t. \quad \inf_{\mu' \in \mathcal{B}}
	\sum_{i=1}^{d} 2 c_i (\mu_i-\mu'_i)^2 \geq 1.
	\end{eqnarray}
	
	In this constrained optimization problem, the constraints set is
	huge because every change of measure $\mu'\in\mathcal{B}(\mu)$ must satisfy 
	\eqref{eq:constraint}. On
	the other side, relaxing some constraints -- or considering only a
	subset of $\mathcal{B}(\mu)$-- simply allows to reach even lower 
	values \footnote{At that point, we may lose the optimality of the finally 
	obtained lower bound but this is a
		price we accept to pay in order to obtain a computable solution. }.

	\begin{figure}
\centering
\includegraphics[width=0.7\linewidth]{figures/LBchangesHoriz}
\caption{Illustration of the various changes of distribution considered in $\mathcal{B}(\mu)$}
\label{fig:changes}
\end{figure}

	
	We distinguish two types of subsets of $\mathcal{B}(\mu)$ illustrated in 
	Figure~\ref{fig:changes}. These changes correspond to two different 
	situations : either an optimal arm is modified and becomes the new best one 
	and then the sparsity of the problem is not modified, or a suboptimal arm 
	becomes the optimal one and one of the best arms must be set to zero
	to preserve the sparse structure of the problem in the 
	considered class of problems. To fix 
	ideas, we have
	$(\cup_{1<i\leq s}
	\mathcal{B}_i(\mu))
	\cup (\cup_{j>s} \mathcal{B}_j(\mu) )\subset \mathcal{B}(\mu)$ where
	\[
	\mathcal{B}_i(\mu) =
	\begin{cases}
	\{\mu' \in \mathcal{S}(d,s) \,\vert\, \mu'_1 = \mu_1,\, \exists
	\gamma
	>0, \mu'_i = \mu_1 + \gamma\} & 1<i\leq s;\\
	\{\mu' \in \mathcal{S}(d,s) \,\vert\, \mu'_1 = \mu_1,\, \exists
	\gamma
	>0, \mu'_i = \mu_1 + \gamma, \, \mu'_j = 0 \} &
	i> s, \, j\leq s.
	\end{cases}
	\]
	Note that for all $i>1$, $\mathcal{B}_i(\mu)$ contains an infinity of models and that in the case of $i>s$, 
	$\mathcal{B}_i(\mu)$ is in fact a union of $s-1$ sets corresponding to the optimal arm that is zeroed to 
	maintain the sparsity of the problem.


	We end up with a finite set of $s-1+(d-s)(s-1)$ constraints that lead to the
	following relaxed version of Eq.~\eqref{eq:opt_problem}: (taking the $\inf$
	over $\gamma >0$ and using $\Delta_j > \mu_1$ for all $j>s$)
	\begin{eqnarray}
	&  & f(\mu)\geq \quad \inf_{c\succeq 0} c_i \Delta_i\\
	s.t. & \quad\forall i\in \{2,...,s\},
	& 2 c_i \Delta_i^2\geq 1;\\
	& \forall i\in \{2,\ldots,s\},\, \forall j\in \{s+1,...d\},  & 2 c_j 
	\mu_1^2+ 2 c_i \mu_i^2 \geq 1\\
	& \forall i\in \{1,\ldots,d\}, & c_i \geq 0
	\end{eqnarray}
	
	This proves the first part of our Theorem.  The technical, computational proof to get the given explicit form for the Lower Bound are deferred to Appendix~\ref{ap:LBproof}. \end{proof}

	\begin{remark}
			This is a linear optimization problem under inequality constraints so 
	there exist algorithmic methods such as the celebrated Simplex 
	algorithm \cite{dantzig2016linear} to compute a numeric solution of it. 
	Nonetheless, in our case, it is 
	possible to give an explicit solution.
	\end{remark}

  	  
% % % OLD AND PROBABLY USELESS:
%CASE WITH ONLY ONE CONSTRAINT ON THE $s$-TH ARM : 
%  	\begin{eqnarray*}
%  	&  & f(\mu)\geq \quad \inf_{c\succeq 0} c_i \Delta_i\\
%  	s.t. & \quad\forall i\in \{2,...,s\},
%  	& 2 c_i \Delta_i^2\geq 1;\\
%  	&  \forall j\in \{s+1,...d\},  & 2 c_j \mu_1^2+ 2 c_i \mu_s^2 \geq 1.
%  	\end{eqnarray*}
%
%This proves the first part of our Theorem. We now solve this problem in order 
%to obtain the given explicit form for the Lower Bound.   	
%We rewrite the argument by taking the constraints into account
%
%\[
%\inf_{c\in \mathbb{N}^d} c_i \Delta_i = \sum_{i=1}^{s-1}\frac{1}{2\Delta_i} + 
%\inf_{c_s \geq 1/\Delta_s^2} c_s \Delta_s+ (d-s)\mu_1\left(\frac{1-2c_s 
%\mu_s^2}{2\mu_1^2}\right)
%\]
%So, we distinguish two cases : 
%\begin{itemize}
%	\item If $\Delta_s -(d-s)\left(\frac{\mu_s^2}{\mu_1}\right) > 0$, $c_s$ 
%must be as small as possible. Then $c_s = 1/2\Delta_s^2$.
%	\item Otherwise, $c_s$ can take a larger value as long as 
%$\left(\frac{1-2c_s \mu_s^2}{2\mu_1^2}\right) >0$. That is, $c_s = \max 
%\{1/2\Delta_s^2; 1/2\mu_s^2\} $.
%\end{itemize}
%
%  	
%  	My conjecture would be the following. For the "best" arms (i.e., $i \leq 
%k^*$), then the number of samples scale as 
%$\max\{\frac{1}{2\Delta_i^2},\frac{1}{2\mu_i^2}\}$ while for the "worse" arms 
%($k^* < i \leq s$), the number of samples scales as 
%$\frac{(1-\lambda)}{2\mu_i^2}$ and the null arms have each a number of samples 
%equal to $\frac{1-\lambda}{2}$ where the numbers $\lambda$ and $k^*$ depends 
%on 
%the different values of $\mu_i$, such that
%  	$$
%  	\sum_{i=k^*+1}^s \frac{\Delta_i}{\mu_i^2} \leq d-s \leq \sum_{i=k^*}^s 
%\frac{\Delta_i}{\mu_i^2}
%  	$$
%	
%  	
%  \end{proof}
%\todov{My conjecture would be the following. For the "best" arms (i.e., $i 
%\leq k^*$), then the number of samples scale as 
%$\max\{\frac{1}{2\Delta_i^2},\frac{1}{2\mu_i^2}\}$ while for the "worse" arms 
%($k^* < i \leq s$), the number of samples scales as 
%$\frac{(1-\lambda)}{2\mu_i^2}$ and the null arms have each a number of samples 
%equal to $\frac{1-\lambda}{2}$ where the numbers $\lambda$ and $k^*$ depends 
%on 
%the different values of $\mu_i$, such that
%$$
%\sum_{i=k^*+1}^s \frac{\Delta_i}{\mu_i^2} \leq d-s \leq \sum_{i=k^*}^s 
%\frac{\Delta_i}{\mu_i^2}
%$$
%Or something like that :)}
%  \begin{corollary}
%  	  	For a sparse bandit problem stated as above, we get the following lower
%  	  	bound on the regret of any uniformly efficient algorithm :
%  	  	
%  	  	\[
%  	  	\liminf_{T\rightarrow \infty} \frac{\operatorname{Reg}(T)}{\log (T)}\geq
%  	  	\sum_{\substack{i\in [s]\\\Delta_i>0}}^{}\frac{1}{2\Delta_i}
%  	  	+ \left(1- \frac{\epsilon^2}{\Delta_s^2} \right)^+
%  	  	\sum_{i=s+1}^{d}\frac{1}{2\Delta_i}
%  	  	\]
%  	  	where $(x)^+ = \max(0,x)$.
%  \end{corollary}
%
%
%    \begin{remark}
%    	The statement of the lower bound allows to quantify somehow how much 
%useful the sparsity information $\epsilon$ is for solving the regret 
%minimization problem.
%    	Basically, we distinguish two cases :
%    	\begin{itemize}
%    		\item If $\epsilon < \Delta_s$, the sparsity information cannot be 
%efficiently used and the regret scales as $\sum_{i=1}^d 1/2\Delta_i$, meaning 
%that the worst arms are costly to explore;
%    		\item If $\epsilon \geq \Delta_s$, the sparsity information is very 
%relevant and can be used to 'eliminate' the bad arms in less than $\log(T)$ 
%exploration
%    		rounds such that the regret due to them vanishes.
%    	\end{itemize}
%    \end{remark}
%    \todoc{nice schema would be appreciated here...}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_colt"
%%% End:


==> combining.tex <==
%!TEX root = main_colt.tex
%


\begin{figure}
  \centering
\begin{tikzpicture}[>=stealth,box/.style={draw,rounded corners}]

 % \node (start) at (-2,0) {start}; 
 \node[box] (round-robin) at (0,0) {round-robin};
 \node (n1) at (4,0) {$\bullet$};
 \node (n2) at (10,0) {$\bullet$};
 \node (n3) at (10,2) {$\bullet$};
 \node[box] (force-log) at (6,3) {force-log};
 \node[box] (UCB) at (6,1.5) {UCB on $\mathcal{K}(t)$};
 \node[box] (ClassicUCB) at (7,-2) {UCB on $[d]$};

 \draw [->] (round-robin)[right] to[bend left]  (n1);
 \draw [->] (n1)[right] to[bend left] node[below]{if $\left|
     \mathcal{J}(t) \right| \neq s$} (round-robin);
 \draw[->] (n1) to node[below]{if $\left| \mathcal{J}(t) \right| =s$} (n2) ;
\draw[->] (n2) to node[right]{sparse enough} (n3);
 \draw[->] (n3) to[bend right] node[above right]{if $\left| \mathcal{K}(t) \right| <s$} (force-log);
 \draw[->] (n3) to[bend right] node[below]{if $\left| \mathcal{K}(t) \right| \geqslant s$} (UCB);
 \draw[->] (force-log) to [bend right] (n1);
 \draw[->] (UCB) to [bend right] (n1);
 \draw[->] (-1.75,0) to (round-robin);
 \draw[->] (n2) to [bend left] node[right]{not sparse enough} (ClassicUCB);
 \draw[->]  (ClassicUCB) to [bend left] (n1);
\end{tikzpicture}
\caption{Combining}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main_colt"
%%% End:

